Extracting Impact Model Narratives from Social Services' Text

Named entity recognition (NER) is an important task in narration extraction. Narration, as a system of stories, provides insights into how events and characters in the stories develop over time. This paper proposes an architecture for NER on a corpus about social purpose organizations. This is the first NER task specifically targeted at social service entities. We show how this approach can be used for the sequencing of services and impacted clients with information extracted from unstructured text. The methodology outlines steps for extracting ontological representation of entities such as needs and satisfiers and generating hypotheses to answer queries about impact models defined by social purpose organizations. We evaluate the model on a corpus of social service descriptions with empirically calculated score.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
